The character map in deformation quantization

The third author recently proved that the Shoikhet-Dolgushev L-infinity-morphism from Hochschild chains of the algebra of smooth functions on manifold to differential forms extends to cyclic chains. Localization at a solution of the Maurer-Cartan equation gives an isomorphism, which we call character map, from the periodic cyclic homology of a formal associative deformation of the algebra of functions to de Rham cohomology. We prove that the character map is compatible with the Gauss-Manin connection, extending a result of Calaque and Rossi on the compatibility with the cap product. As a consequence, the image of the periodic cyclic cycle 1 is independent of the deformation parameter and we compute it to be the A-roof genus of the manifold. Our results also imply the Tamarkin-Tsygan index Theorem.

==> PSMondisk_v4.tex <==

\subsection{Relation to the Poisson sigma model on the disk}
The first two authors introduced in \cite{CF} the equivariant Poisson sigma model on the disk. 
Assume that the manifold $M$ is compact and oriented with volume form $\Omega$.
Then one obtains an $L_\infty$-morphism 
\[
 \mV_{PSM,orig}: (C_\bullet(A,A)[[u]],b+uB) \to (T^\bullet(M)[[u]], u \dv_\Omega).
\]
of modules over $(T^\bullet(M)[[u]], u \dv_\Omega, \co{\cdot}{\cdot}_S)$. Locally, this is given by
vacuum expectation values of the Poisson sigma model on the disk with trivial Poisson structure and its globalization
is described in \cite{CFW}, where it is also shown that
\begin{equation}\label{e:PSMorig}
 \mV^{*}_{PSM,n}(\gamma_1,\dots,\gamma_n)(\gamma)(a_0,\dots,a_m)
:=
\iota_{\mV_{PSM,orig,n+1}(\gamma_1,\dots,\gamma_m,u\gamma;a_0,\dots,a_m)}\Omega,
\end{equation}
for any multivector fields $\gamma, \gamma_1,\dots,\gamma_n$ and smooth functions $a_0,\dots,a_m$,
is a quasi\ndash isomorphism of $L_\infty$-modules:
\[
 \mV^*_{PSM} : (T^\bullet(M)[u],u\dv) \cong (VT^\bullet(M)[u], ud) \to (E_{norm}^\bullet[u], \nabla+b+uB).
\]
The nonequivariant Poisson sigma model on the disk produces the $u=0$ term only.

This morphism is the adjoint (in a suitable sense) to the Shoikhet--Dolgushev morphism $\mV$ above. Using the volume form $\Omega$,
one can define nondegenerate pairings $\skp{\cdot}{\cdot}$ between multivector fields and differential forms and Hochschild chains and cochains, such that
\begin{equation}\label{e:PSMSD}
\begin{split}
\skp{\mV_{PSM,n}^*(\gamma_1,\dots,\gamma_n)(\gamma)}{(a_0, \dots, a_m)} 
&:= \int_M \mV_{PSM,n}^*(\gamma_1,\dots,\gamma_n)(\gamma)(a_0,\dots, a_m) \\
&= \pm \skp{\gamma}{\mV_n(\gamma_1,\dots,\gamma_n; a_0, \dots, a_m)} \\
&:= \pm \int_M \left( \iota_\gamma \mV_n(\gamma_1,\dots,\gamma_n; a_0, \dots, a_m) \right) \Omega.
\end{split}
\end{equation}
%\begin{equation}\label{e:PSMSD}
%\mV_{PSM,n}^*(\gamma_1,\dots,\gamma_n)(\gamma)(a_0,\dots, a_m) = \pm \skp{\gamma}{\mV_n(\gamma_1,\dots,\gamma_n; a_0, \dots, a_m)}.
%\end{equation}

\newcommand{\Tr}{\operatorname{Tr}_{\pi,\Omega}}
\newcommand{\vev}[1]{{\left\langle\;{#1}\;\right\rangle}_{\pi,\Omega}}
Let now $\pi$ be a unimodular Poisson structure with $\dv_\Omega\pi=0$.\footnote{A Poisson structure is called unimodular if its divergence with respect to some (and hence every) volume form is a Hamiltonian vector field. If this is the case, rescaling the volume form by the exponential of the Hamiltonian function yields a volume form with respect to which the Poisson structure is divergence-free. If $\{\ ,\ \}$ denotes the Poisson bracket, then the last condition is equivalent to $\int_M\{f,g\}\,\Omega=0$, $\forall f,g$.}
Then the perturbative partition function of the Poisson sigma model is defined as\footnote{The formal parameter $\hbar$ appearing here
is actually $\sqrt{-1}$ times the physical Planck constant appearing in the Poisson sigma model.}
\[
Z_{PSM}(\pi,\Omega):=\sum_{n=0}^\infty \frac{\hbar^n}{n!}\,\int_M \iota_{\mV_{PSM,orig,n}(\pi,\dots,\pi;1)}\Omega.
\]
More generally, one can define the (nonnormalized) expectation value of $f\in C^\infty(M)[[\hbar]]$ by putting $f$ instead of $1$ in the above
formula. In \cite{CF} it was shown that locally this defines a trace for the Kontsevich star product, so we write
\[
\Tr f:=\sum_{n=0}^\infty \frac{\hbar^n}{n!}\, \int_M \iota_{\mV_{PSM,orig,n}(\pi,\dots,\pi;f)}\Omega.
\]
\begin{proposition}
Let $M$ be a compact manifold, $\pi$ a Poisson structure and $\Omega$ a volume form on $M$ with $\dv_\Omega\pi=0$. Then
\begin{enumerate}
\item $\Tr$ is a trace for the star product $\mathcal U_0^\pi$.
\item 
\[
Z_{PSM}(\pi,\Omega)=\Tr1=\int_M \hat{A} \wedge e^{\hbar \iota_\pi}\Omega.
\]
\end{enumerate}
\end{proposition}
\begin{proof}
For a cyclic chain $(f_0,\dots, f_m)$, we set
\[
\vev{(f_0,\dots, f_m)}:=
\sum_{n=0}^\infty \frac{\hbar^n}{n!}\, \int_M \iota_{\mV_{PSM,orig,n}(\pi,\dots,\pi;f_0,\dots,f_m)}\Omega.
\]
In particular $\Tr f=\vev f$. To prove the first statement in the Proposition, we now observe that 
$\vev{(b_*+uB)(f, g)}=0$ $\forall f,g$ 
since $\mV_{PSM,orig}$ is an $L_\infty$\ndash morphism and $\dv_\Omega\pi=0$. By construction\footnote{In the formula we select
the component of  $\mV_{PSM,orig}$ which is a zero-vector field, i.e., a function. This is locally given by graphs in \cite{CF} with no white
vertices. The contributions on $(1, f, g)$ is then zero since in the graphs only bivector fields (the local expression of $\pi$) and vector fields (coming from the globalization) appear.}
we also have
$\vev{(1, f, g)}=0$.

To prove the second statement, we use equations \eqref{e:PSMorig} and \eqref{e:PSMSD} and obtain
\[
Z_{PSM}:= Vol(M) + \int_0^\hbar \skp{\mV_{PSM}^{*,\pi}(\frac{1}{u}\pi)}{1}\; d\hbar
= Vol(M) - \int_0^\hbar \frac{1}{u} \skp{\pi}{\mV^\pi(1)} \;d\hbar,
\]
where $\int_0^\hbar\dots d\hbar$ denotes formal integration with respect to $\hbar$ and $\mV_{PSM}^{*,\pi}$ denotes the $L_\infty$\ndash morphism
twisted by $\pi$.
By the main results of this paper, we finally get
\begin{align*}
Z_{PSM} &= Vol(M) - \int_0^\hbar \frac{1}{u} \skp{\pi}{e^{-\hbar \iota_\pi/u}\hat{A}_u}\;d\hbar
\\&=  Vol(M) - \int_0^\hbar \frac{1}{u} \int_M (\iota_\pi e^{-\hbar \iota_\pi/u}\hat{A}_u)\Omega \;d\hbar
\\&= \int_M \hat{A}_u \wedge e^{\hbar \iota_\pi/u}\Omega 
=  \int_M \hat{A} \wedge e^{\hbar \iota_\pi}\Omega.
\end{align*}
\end{proof}
 The formula for the trace of one is the same as the one found by Tamarkin and Tsygan in \cite{TamarkinT}.




